Monte-Carlo Tree Search for Efficient Visually Guided Rearrangement Planning

We address the problem of visually guided rearrangement planning with many movable objects, i.e., finding a sequence of actions to move a set of objects from an initial arrangement to a desired one, while relying on visual inputs coming from an RGB camera. To do so, we introduce a complete pipeline relying on two key contributions. First, we introduce an efficient and scalable rearrangement planning method, based on a Monte-Carlo Tree Search exploration strategy. We demonstrate that because of its good trade-off between exploration and exploitation our method (i) scales well with the number of objects while (ii) finding solutions which require a smaller number of moves compared to the other state-of-the-art approaches. Note that on the contrary to many approaches, we do not require any buffer space to be available. Second, to precisely localize movable objects in the scene, we develop an integrated approach for robust multi-object workspace state estimation from a single uncalibrated RGB camera using a deep neural network trained only with synthetic data. We validate our multi-object visually guided manipulation pipeline with several experiments on a real UR-5 robotic arm by solving various rearrangement planning instances, requiring only 60 ms to compute the plan to rearrange 25 objects. In addition, we show that our system is insensitive to camera movements and can successfully recover from external perturbations. Supplementary video, source code and pre-trained models are available at https://ylabbe.github.io/rearrangement-planning.

==> Makefile <==
TEX_FILES = root.tex introduction.tex related_work.tex mcts.tex vision.tex experiments.tex conclusion.tex
ABSTRACT_TEX_FILES = extended.tex introduction_short.tex mcts_short.tex experiments_short.tex vision_short.tex
FIGURE_NAMES = teaser.pdf high_level_2.pdf configs.pdf goal-param.pdf visual_system.pdf train_images.pdf mcts.pdf test_n_objects.pdf plot_variable_n_objects.pdf src_tgt_pipeline.pdf
GS_EBOOK = teaser.pdf
GS_PRINTER = src_tgt_pipeline.pdf test_n_objects.pdf train_images.pdf
all:
	latexmk -pdf -quiet root
arxiv:
	mkdir -p arxiv
	cp root.bbl $(TEX_FILES) ieeeconf.cls ./arxiv
	# remove comments
	$(foreach name,$(TEX_FILES),latexpand --empty-comments \
		$(name) | sed '/^\s*%/d' > ./arxiv/$(name);)
	mkdir -p ./arxiv/figures
	$(foreach name,$(FIGURE_NAMES),cp ./figures/$(name) ./arxiv/figures/$(name);)
	$(foreach name,$(GS_EBOOK),gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/ebook -dNOPAUSE -dQUIET -dBATCH \
		-sOutputFile=arxiv/figures/$(name) figures/$(name);)
	$(foreach name,$(GS_PRINTER),gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.4 -dPDFSETTINGS=/printer -dNOPAUSE -dQUIET -dBATCH \
		-sOutputFile=arxiv/figures/$(name) figures/$(name);)
	zip -r arxiv.zip arxiv/*
clean:
	latexmk -c root
	rm -rf ./arxiv
extended_abstract:	arxiv
	cp -r ./arxiv ./extended_abstract
	cp $(ABSTRACT_TEX_FILES) IEEEtran.cls ./extended_abstract


